TAP4LLM: Table Provider on Sampling, Augmenting, and Packing Semi-structured Data for Large Language Model Reasoning

Table reasoning tasks have shown remarkable progress with the development of large language models (LLMs), which involve interpreting and drawing conclusions from tabular data based on natural language (NL) questions. Existing solutions mainly tested on smaller tables face scalability issues and struggle with complex queries due to incomplete or dispersed data across different table sections. To alleviate these challenges, we propose TAP4LLM as a versatile pre-processor suite for leveraging LLMs in table-based tasks effectively. It covers several distinct components: (1) table sampling to decompose large tables into manageable sub-tables based on query semantics, (2) table augmentation to enhance tables with additional knowledge from external sources or models, and (3) table packing & serialization to convert tables into various formats suitable for LLMs' understanding. In each module, we design and compare several common methods under various usage scenarios, aiming to shed light on the best practices for leveraging LLMs for table-reasoning tasks. Our experiments show that our method improves LLMs' reasoning capabilities in various tabular tasks and enhances the interaction between LLMs and tabular data by employing effective pre-processing.

==> misc/acknowledgement.tex <==
\section*{Acknowledgements}

==> misc/author.tex <==

\author
{
    \IEEEauthorblockN
    {
        Yuan Sui\IEEEauthorrefmark{1}\printfnsymbol{1},
        \thanks{
            \printfnsymbol{1} This work was mostly done in Microsoft Research Asia as a research intern at DKI Group, and completed in NUS.
        }
        Mengyu Zhou\IEEEauthorrefmark{2}\printfnsymbol{2},
        \thanks{
            \printfnsymbol{2} Corresponding author.
        }
        Jiaru Zou\IEEEauthorrefmark{3}\printfnsymbol{1},
	Xinyi He\IEEEauthorrefmark{4}\printfnsymbol{1},
        Lun Du\IEEEauthorrefmark{2},
        Shi Han\IEEEauthorrefmark{2},
        Dongmei Zhang\IEEEauthorrefmark{2}
        }
	\IEEEauthorblockA{
            \IEEEauthorrefmark{1}National University of Singapore, 
            \IEEEauthorrefmark{2}Microsoft, 
            \IEEEauthorrefmark{3}University of Illinois Urbana-Champaign, 
            \IEEEauthorrefmark{4}Xi'an Jiaotong University, \\ 
        \texttt{\href{mailto:yuan.sui@u.nus.edu}{yuan.sui@u.nus.edu}}, 
        \texttt{\href{mailto:jiaruz2@illinois.edu}{jiaruz2@illinois.edu}}, \texttt{\href{mailto:hxyhxy@stu.xjtu.edu.cn}{hxyhxy@stu.xjtu.edu.cn}},\\
        \texttt{\{\href{mailto:mezho@microsoft.com}{mezho}, \href{mailto:lun.du@microsoft.com}{lun.du}, \href{mailto:shihan@microsoft.com}{shihan}, \href{mailto:dongmeiz@microsoft.com}{dongmeiz}\}@microsoft.com}
    }
  }

==> misc/author_acm.tex <==
% \author{Ben Trovato}
% \affiliation{%
%   \institution{Institute for Clarity in Documentation}
%   \streetaddress{P.O. Box 1212}
%   \city{Dublin}
%   \state{Ireland}
%   \postcode{43017-6221}
% }
% \email{trovato@corporation.com}

% \author{Lars Th{\o}rv{\"a}ld}
% \orcid{0000-0002-1825-0097}
% \affiliation{%
%   \institution{The Th{\o}rv{\"a}ld Group}
%   \streetaddress{1 Th{\o}rv{\"a}ld Circle}
%   \city{Hekla}
%   \country{Iceland}
% }
% \email{larst@affiliation.org}

% \author{Valerie B\'eranger}
% \orcid{0000-0001-5109-3700}
% \affiliation{%
%   \institution{Inria Paris-Rocquencourt}
%   \city{Rocquencourt}
%   \country{France}
% }
% \email{vb@rocquencourt.com}

% \author{J\"org von \"Arbach}
% \affiliation{%
%   \institution{University of T\"ubingen}
%   \city{T\"ubingen}
%   \country{Germany}
% }
% \email{jaerbach@uni-tuebingen.edu}
% \email{myprivate@email.com}
% \email{second@affiliation.mail}

% \author{Wang Xiu Ying}
% \author{Zhe Zuo}
% \affiliation{%
%   \institution{East China Normal University}
%   \city{Shanghai}
%   \country{China}
% }
% \email{firstname.lastname@ecnu.edu.cn}

% \author{Donald Fauntleroy Duck}
% \affiliation{%
%   \institution{Scientific Writing Academy}
%   \city{Duckburg}
%   \country{Calisota}
% }
% \affiliation{%
%   \institution{Donald's Second Affiliation}
%   \city{City}
%   \country{country}
% }
% \email{donald@swa.edu}

% IEEE
% \author
% {
%     \IEEEauthorblockN
%     {
%         Yuan Sui\IEEEauthorrefmark{1}\printfnsymbol{1},
%         \thanks{
%             \printfnsymbol{1} This work was mostly done in Microsoft Research Asia as a research intern at DKI Group, and completed in NUS.
%         }
%         Mengyu Zhou\IEEEauthorrefmark{2}\printfnsymbol{2},
%         \thanks{
%             \printfnsymbol{2} Corresponding author.
%         }
%         Jiaru Zou\IEEEauthorrefmark{3},
% 	Xinyi He\IEEEauthorrefmark{4},
%         Lun Du\IEEEauthorrefmark{2},
%         Shi Han\IEEEauthorrefmark{2},
%         Dongmei Zhang\IEEEauthorrefmark{2}
%         }
% 	\IEEEauthorblockA{
%             \IEEEauthorrefmark{1}National University of Singapore, 
%             \IEEEauthorrefmark{2}Microsoft, 
%             \IEEEauthorrefmark{3}University of Illinois Urbana-Champaign, 
%             \IEEEauthorrefmark{4}Xi'an Jiaotong University, \\ 
%         \texttt{\href{mailto:yuan.sui@u.nus.edu}{yuan.sui@u.nus.edu}}, 
%         \texttt{\href{mailto:jiaruz2@illinois.edu}{jiaruz2@illinois.edu}}, \texttt{\href{mailto:hxyhxy@stu.xjtu.edu.cn}{hxyhxy@stu.xjtu.edu.cn}},\\
%         \texttt{\{\href{mailto:mezho@microsoft.com}{mezho}, \href{mailto:lun.du@microsoft.com}{lun.du}, \href{mailto:shihan@microsoft.com}{shihan}, \href{mailto:dongmeiz@microsoft.com}{dongmeiz}\}@microsoft.com}
%     }
%   }

\author{Yuan Sui}
\authornote{Yuan, Jiaru and Xinyi made their contributions during their internship at Microsoft.}
%\authornote{Yuan Sui made the majority of his contributions during his internship at Microsoft Research Asia, and later completed it at NUS. Jiaru Zou and Xinyi He made their contributions during their internship at Microsoft.}
% This work was mostly done in Microsoft Research Asia as a research intern at DKI Group, and completed in NUS.}
\affiliation{
    \institution{National University of Singapore}
    % \country{Singapore}
    \country{} 
}
\email{yuan.sui@u.nus.edu}

\author{Jiaru Zou}
\authornotemark[1]
\affiliation{
    \institution{University~of~Illinois~Urbana-Champaign}
    % \country{Champaign, IL, USA}
}
\email{jiaruz2@illinois.edu}

\author{Mengyu Zhou}
\authornote{Corresponding author.}
\affiliation{
    \institution{Microsoft}
    % \country{Beijing, China}
    \country{} 
}
\email{mezho@microsoft.com}


\author{Xinyi He}
\authornotemark[1]
\affiliation{
    \institution{Xi'an Jiaotong University}
    % \country{Xi'an, China}
    \country{} 
}
\email{hxyhxy@stu.xjtu.edu.cn}

\author{Lun Du}
\affiliation{
    \institution{Microsoft}
    % \country{Beijing, China}
    \country{} 
}
\email{lun.du@microsoft.com}

\author{Shi Han, Dongmei Zhang}
\affiliation{
    \institution{Microsoft}
    % \country{Beijing, China}
    \country{} 
}
\email{{shihan, dongmeiz}@microsoft.com}


% \author{Dongmei Zhang}
% \affiliation{
%     \institution{Microsoft}
%     % \country{Beijing, China}
% }
% \email{dongmeiz@microsoft.com}


==> sources/2-preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

\begin{figure*} 
    \centering
    \includegraphics[width=1\linewidth]{sources/figs/TableProvider-Framework-v5.pdf}
    \caption{\small{\ours{} Framework for Tabular Data. Noted that the ``table sync'' refers to the application (such as Excel Copilot) keeps its table data in sync with the table manager. The table manager acts as an intermediary, managing the data that is either stored locally in a cache or accessed through a database connection. This syncing process is crucial for ``interactive table reasoning'' and for maintaining data integrity. The implication of this syncing process is further discussed in \refsec{sec:interactive_table_reasoning}.}}
    \label{fig:table_provider_framework}
\end{figure*}

\textbf{Table Reasoning Tasks}.
Each instance in table-based reasoning consists of a table $T$, a natural language question $Q$, and an answer $A$. Specifically, table $T$ is defined as $T=\left\{v_{i, j} \mid i\leq\operatorname{R}_T, j\leq\operatorname{C}_T\right\}$, containing $R_T$ rows and $C_T$ columns. The content of the cell in the $i$-th row and $j$-th column is represented by $v{i, j}$. A question $Q$ is a sequence of $n$ tokens: $Q=\{q_1, q_2, q_3, \cdots, q_n\}$.
In this paper, our primary focus is on two distinct table-based reasoning tasks, table-based fact verification (TFV) and table-based question answering (TQA). In TFV, the answer $A$ is a boolean value in $\{0,1\}$, indicating the veracity of the input statement (where $1$ means the statement is entailed by the given table, and $0$ means the statement is refuted by the given table). In TQA, the answer is a sequence of natural language tokens represented as $A=\{a_1, a_2, a_3, \cdots, a_n\}$ corresponding to the posed question.
For our experiments, all tables first undergo table sampling and table augmentation by our proposed method and then are serialized into a sequence by table packing and serialization. Note that various serialization methods have already been explored in our previous work~\cite{model_structure_LLM}. Detailed implementation specifics are provided in Section~\refsec{sec:table_packing_serialization}.



% \notableparagraph{Table Serialization Methods}
% Serializing tables into a sequence format is an essential step when adapting to the masked language modeling objectives of LLMs~\cite{hegselmann2023tabllm}. 
% One straightforward serialization approach is to process tables row-by-row. 
% This method has been adopted by numerous studies, including TaPas~\cite{model_tapas}, MATE~\cite{model_mate}, TableFormer~\cite{model_tableformer}, TUTA~\cite{model_tuta}, and TURL~\cite{model_turl}. In TaPEx~\cite{model_tapex}, the table is linearized by rows; however, it incorporates special tokens such as $<$HEAD$>$ and $<$ROW$>$ to signify headers and rows, respectively.
% Similarly, TABBIE~\cite{model_tabbie} serializes tables in both row-wise and column-wise manners. Meanwhile, TableGPT~\cite{model_tablegpt} uses a template-based method to serialize the attribute-value pair within each table record. Throughout the literature, a plethora of thoughtfully designed sequence serialization methods have been presented, establishing standard practices in table serialization~\cite{model_tapex,model_tapas,model_tuta,model_formlm, model_unifiedSKG,model_uniSAr}.

\textbf{Challenges with Long Sequences in LLMs}.
Most LLMs struggle with long sequences due to the quadratic complexity of self-attention mechanisms~\cite{model_selfattention, survey_effecienttransformer}.  It's important to note that the maximum sequence length of commonly used LLMs, such as gpt-3.5-turbo-16k~\cite{zotero-3375}, is limited to 16k tokens. This limit becomes especially problematic when dealing with structured data, which typically consists of various components and causes significant memory and computational challenges. 
Solutions like Tapex~\cite{model_tapex} and Tapas~\cite{model_tapas} utilize a simple truncation approach based on the table's sequence length. However, these methods exhibit the shortcomings of excluding important data and disrupting the whole table structure.
In our work, we introduce specific constraints for the LLMs' call requests. For example, to avoid structural disruptions from truncation, we use a \textit{``token allocation''} strategy to estimate the token capacity and initiate the sampling functions (explained in Section~\refsec{sec:table_sampling}) when the table's token count surpasses a certain threshold.

% \textbf{Neuro-Symbolic Functions \& Metadata Analysis}.
% Neuro-symbolic method is a specialized approach in Deep Learning (DL) that combines neural and symbolic methodologies~\cite{hitzler2022}. 
% % The term \textit{neural} refers to approaches based on deep neural networks, which have achieved remarkable breakthroughs in the past decade and ignited the prevailing enthusiasm for AI. Conversely, \textit{symbolic} relies on the explicit representation of knowledge via formal languages—including formal logic—and the algorithmic manipulation of symbolic entities to attain desired outcomes. 
% In this work, we use Metadata Analysis~\cite{he2023anameta}, a neuro-symbolic method based on a transformer architecture~\cite{model_selfattention}, to generate metadata essential for table analysis.
% Such metadata serves as an explicit representation of formally organized background knowledge. An example of this is the binary metadata classification for column types, known as dimension and measure\footnote{A measure is a table field consisting of numerical data that you can calculate, such as 'Price' and 'Discount'. Conversely, a dimension is a field that offers categorical information used for filtering, grouping, and labeling, such as the 'Product Name' and 'Category'. It's important to correctly classify fields as measures or dimensions because they dictate the operations you can perform on the data, affecting the accuracy and relevance of the analysis.}.
% Furthermore, various LLM-centric toolsets have been developed to facilitate: (\romannumeral1) integration of LLMs with diverse data sources, and (\romannumeral2) dynamic interactions of LLMs with their surroundings. 
% We select some of symbolic functions from the toolsets as our agents for table augmentation, including Langchain~\cite{langchain}, Semantic Kernel~\cite{semantic-kernel}, \etc.

==> sources/5-discussion.tex <==
\section{Implementation Details}
\label{sec:discussion}

To achieve the interactive table reasoning,
\label{sec:interactive_table_reasoning}
\ours{} proposes the ``table sync'' to ensure that applications, such as Excel Copilot, maintain their table data in synchronization with the table manager. The table manager acts as a go-between, managing the data that is either stored locally in a cache or accessed through a database connection. Specifically, when changes are made to the data within the application, those changes must be reflected in the table manager for any operation performance, such as sampling, augmentation, and packing. Conversely, if changes are made within the table manager, the changed data should be updated in the application as well.

This syncing process is essential for maintaining data integrity and ensuring that all components of the system are kept up-to-date. This is especially beneficial when the data is being used to generate prompts for a large language model, as it allows for accurate data processing, querying, and analysis. By having the most current and relevant information, the model can provide accurate and reliable responses.

(2) \textit{Table Cleansing}:
\label{sec:table_cleansing}
Table cleansing is an independent step in tabular data prepossessing, especially when dealing with hierarchical tables. In the context of fine-grained in-context learning, where pre-trained generated model has to discern and process intricate patterns and relationships within datasets. The importance of clean and standardized tables cannot be overstated for two reasons: (1) Dirty or unorganized tabular data can mislead the models and impair the model's performance; (2) Cleansed tables ensure uniformity, making them easier to compare, merge, or use in subsequent operations. For example, imagine a financial analyst case aiming to forecast a company's stock price based on historical data. The corresponding table contains daily stock prices, trading volumes, and various financial indicators. If there are any missing certain values for certain days, or duplicate entries due to system glitches. Such inconsistencies may dramatically affect the forecasting performance. For instance, it might suggest a non-trading day or a sudden drop in stock price.
Specially, the formal definition of table cleansing is: Given a table $T$ consisting of rows $R_T$ and columns $C_T$, table cleansing transforms $T$ into $T'$ such that:

(a) \textit{Cell and column name completeness}: For every cell $c_{i,j}$ in $T$ where $i \in R_T$ and $j \in C_T$, if $c_{i, j}$ has a missing or null value, it is filled using contextual information (\ie, use the corresponding entire column $C_j$ of cell $c_{i,j}$ as the context). We utilize a separate ``CallLLM" system $g(\cdot)$ to call a pre-trained language model to synthesize the missing value. The processing can be formulated as $c_{i,j}=g(C_j)$. This ensures that gaps in the data don't lead to misleading interpretations or missed patterns.

(b) \textit{Duplicate data points removal}: For every pair of rows $r_m$, $r_n$ and pair of columns $c_p$, $c_q$ in $T$, if $r_m=r_n$ or $c_p=c_q$ respectively, one from the pair is removed to eliminate duplication.

(c) \textit{Format consistency}: For every cell $c_{i,j}$ in $T$, the value conforms to a specific format, unit, or pattern.

==> sources/tables/cell_selection.tex <==
% \begin{table*}[htbp]
%   \centering
%   \caption{Comparative results of cell selection functions. We use query-based sampling as the baseline.}
%     % Table generated by Excel2LaTeX from sheet 'Sheet3'
%     \begin{tabular}{ccccccc}
%     \toprule
%     Method & SQA   & FEVEROUS & TabFact & HybridQA & ToTTo & Spider\\
%     \midrule
%     baseline & 28.32\% & 63.32\% & 59.80\% & 24.32\% & 49.14\% & 80.27\% \\
%     \midrule
%     LLM-based & 31.59\% ($\uparrow\textbf{3.27}\%$) & 64.12\% ($\uparrow\textbf{0.80}\%$) & 62.32\% ($\uparrow\textbf{2.52}\%$) & 26.24\% ($\uparrow\textbf{1.92}\%$) & 53.21\% ($\uparrow\textbf{4.07}\%$) & 80.48\% ($\uparrow\textbf{0.21}\%$)\\
%     Heuristics-based & 29.59\% ($\uparrow1.27\%$) & 63.72\% ($\uparrow0.40\%$) & 61.58\% ($\uparrow1.78\%$) & 25.24\% ($\uparrow0.92\%$) & 51.21\% ($\uparrow2.07\%$) & 80.33\% ($\uparrow0.06\%$)\\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:cell-selection}%
% \end{table*}%

\begin{table*}[htbp]
  \centering
  \caption{\small{Comparative results of cell selection functions. We use query-based sampling as the baseline and GPT-3.5-burbo for LLM-based function.}}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccccccccc}
    \toprule
    \multirow{2}[4]{*}{Methods} & \multicolumn{2}{c}{SQA} & \multicolumn{2}{c}{FEVEROUS} & \multicolumn{2}{c}{TabFact} & \multicolumn{2}{c}{HybridQA} & \multicolumn{2}{c}{ToTTo} & \multicolumn{2}{c}{Spider}\\
    \cmidrule{2-13}      & Acc   & Delta & Acc   & Delta & Acc   & Delta & Acc   & Delta & BLEU-4 & Delta & Acc   & Delta\\
    \midrule
    LLM-based & 31.59\% & \textbf{3.27\%} & 64.12\% & \textbf{0.80\%} & 62.32\% & \textbf{2.52\%}& 26.24\% & \textbf{1.92\%} & 53.21\% & \textbf{4.07\%} & 80.48\% & \textbf{0.21\%}\\
    Heuristics-based & 29.59\% &1.27\% & 63.72\% &0.40\% & 61.58\% &1.78\% & 25.24\%& 0.92\% & 51.21\% & 2.07\% & 80.33\% & 0.06\%\\
    \bottomrule
    \end{tabular}%
  }
  \label{tab:cell-selection}%
\end{table*}



% \begin{table*}[htbp]
%   \centering
%   \caption{Comparative results of cell selection functions. We use query-based sampling as the baseline.}
%     % Table generated by Excel2LaTeX from sheet 'Sheet3'
%     \begin{tabular}{ccccccc}
%     \toprule
%     Method & SQA   & FEVEROUS & TabFact & HybridQA & ToTTo & Spider\\
%     \midrule
%     baseline & 28.32\% & 63.32\% & 59.80\% & 24.32\% & 49.14\% & 80.27\% \\
%     \midrule
%     LLM-based & 31.59\% ($\uparrow\textbf{3.27}\%$) & 64.12\% ($\uparrow\textbf{0.80}\%$) & 62.32\% ($\uparrow\textbf{2.52}\%$) & 26.24\% ($\uparrow\textbf{1.92}\%$) & 53.21\% ($\uparrow\textbf{4.07}\%$) & 80.48\% ($\uparrow\textbf{0.21}\%$)\\
%     Heuristics-based & 29.59\% ($\uparrow1.27\%$) & 63.72\% ($\uparrow0.40\%$) & 61.58\% ($\uparrow1.78\%$) & 25.24\% ($\uparrow0.92\%$) & 51.21\% ($\uparrow2.07\%$) & 80.33\% ($\uparrow0.06\%$)\\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:cell-selection}%
% \end{table*}%

==> sources/tables/knowledge-classification.tex <==
\begin{table*}[htbp]
\centering
\caption{Knowledge Type Classification}
\label{tab:knowledge-classification}
\resizebox{\linewidth}{!}{
\begin{tabular}{|p{2.5cm}|p{5cm}|l|}
\hline
\textbf{Knowledge Type/Name} & \textbf{Description} & \textbf{Symbolic Function} \\
\hline
Commonsense Knowledge & General knowledge about the world that is commonly understood and shared among people. It helps in understanding implicit information and making logical inferences. & \texttt{commonsense\_augmentation(table)} \\
\hline
Domain Knowledge & Specific knowledge about a particular field or domain. It provides specialized information and context relevant to the subject matter of the table. & \texttt{domain\_augmentation(table)} \\
\hline
Structural Knowledge & Knowledge about the structure and organization of the table, including column names, data types, and relationships between columns. It helps in interpreting the table's schema and extracting meaningful insights. & \texttt{structural\_augmentation(table)} \\
\hline
Analytical Knowledge & Knowledge about analytical techniques and methods to process and analyze tabular data. It includes statistical measures, data transformations, and visualization approaches that aid in gaining insights from the table. & \texttt{analytical\_augmentation(table)} \\
\hline
\end{tabular}}
\end{table*}


==> sources/tables/token_allocation.tex <==
\begin{table}[htbp]
  \centering
  \caption{Token Allocation. T:A refers to the table token limit portion vs. the augmentation token limit portion.}
    \begin{tabular}{cc}
    \toprule
    T:A Portion & tabfact \\
    \midrule
    9:1   & \cellcolor[rgb]{ .988,  .988,  1}52.10\% \\
    8:2   & \cellcolor[rgb]{ .776,  .906,  .82}53.78\% \\
    7:3   & \cellcolor[rgb]{ .573,  .82,  .643}55.40\% \\
    6:4   & \cellcolor[rgb]{ .525,  .8,  .6}55.78\% \\
    5:5   & \cellcolor[rgb]{ .416,  .757,  .506}56.65\% \\
    4:6   & \cellcolor[rgb]{ .388,  .745,  .482}56.84\% \\
    3:7   & \cellcolor[rgb]{ .824,  .922,  .859}53.42\% \\
    \bottomrule
    \end{tabular}
  \label{tab:token-allocation}
\end{table}

